Guarded Traced Categories

Notions of guardedness serve to delineate the admissibility of cycles, e.g. in recursion, corecursion, iteration, or tracing. We introduce an abstract notion of guardedness structure on a symmetric monoidal category, along with a corresponding notion of guarded traces, which are defined only if the cycles they induce are guarded. We relate structural guardedness, determined by propagating guardedness along the operations of the category, to geometric guardedness phrased in terms of a diagrammatic language. In our setup, the Cartesian case (recursion) and the co-Cartesian case (iteration) become completely dual, and we show that in these cases, guarded tracedness is equivalent to presence of a guarded Conway operator, in analogy to an observation on total traces by Hasegawa and Hyland. Moreover, we relate guarded traces to unguarded categorical uniform fixpoint operators in the style of Simpson and Plotkin. Finally, we show that partial traces based on Hilbert-Schmidt operators in the category of Hilbert spaces are an instance of guarded traces.

==> defslmcs.tex <==

%
\let\theorem\relax
\let\endtheorem\relax
\let\corollary\relax
\let\endcorollary\relax
\let\lemma\relax
\let\endlemma\relax
\let\proposition\relax
\let\endproposition\relax
\let\assumption\relax
\let\endassumption\relax

\let\remark\relax
\let\endremark\relax
\let\example\relax
\let\endexample\relax
\let\defintion\relax
\let\enddefinition\relax
\let\example\relax
\let\endexample\relax

\newenvironment{theorem}{\begin{thm}}{\end{thm}}
\newenvironment{corollary}{\begin{cor}}{\end{cor}}
\newenvironment{lemma}{\begin{lem}}{\end{lem}}
\newenvironment{proposition}{\begin{prop}}{\end{prop}}
\newenvironment{assumption}{\begin{asm}}{\end{asm}}

\newenvironment{remark}{\begin{rem}}{\end{rem}}
\newenvironment{example}{\begin{exa}}{\end{exa}}
\newenvironment{definition}{\begin{defi}}{\end{defi}}




==> partial-hs.tex <==
Given $a\in V$, let $\tau_a:X\to V\tensor X$ be the operator sending $x\in X$ to 
$a\tensor x$.
\begin{definition}[Parametrized Hilbert-Schmidt operators]\label{defn:p-hs}
We call a bounded linear operator $f:V\tensor X\to Y$ \emph{parametrized Hilbert-Schmidt} 
if (i) for any $a\in V$, the operator $f\comp\tau_a:X\to Y$ is Hilbert-Schmidt and (ii) there
exists a real number $c$ such that $\norm{f\comp\tau_a}_2\leq c \norm{a}$ for any $a\in V$.
Let us denote by $HS_V(X,Y)$ the space of all parametrized Hilbert-Schmidt operators
$f:V\tensor X\to Y$.
\end{definition}
%
Clearly, $f\in\HS(X,Y)$ iff $f\comp \upsilon_X^\mone\in\HS_I(X,Y)$.
Condition~(ii) of Definition~\ref{defn:p-hs} requires in other words that the linear 
operator $\curry(f)$ from~$V$ to $\HS(X,Y)$ sending $a\in V$ to $f\comp\tau_a$ is bounded.
Hence we obtain an embedding $\curry: \HS_V(X,Y)\to\Hom(V, \HS(X,Y))$, which, according
to Proposition~\ref{prop:hs-nucl} turns into an isomorphism if $V=I$. 
%
%
\begin{lemma}\label{lem:q-hs-nat}
%
Given $f:V\tensor X\to Y$, $g:V'\to V$, $h:X'\to X$ and $u:Y\to Y'$, 
%
\begin{enumerate}
 \item if $f\in \HS_V(X,Y)$ then $u\comp f\comp (g\tensor h)\in \HS_{V'}(X',Y')$;
 \item if $f\in \HS_V(X,Y)$ and $g\in \HS(V',V)$ then $u\comp f\comp (g\tensor h)\in \HS(X'\tensor V',Y')$;
 \item if $h\in \HS(X', X)$ then $u\comp f(g\tensor h)\in \HS_V(X',Y)$.
%
\end{enumerate} 
\end{lemma}
\begin{proof}
Observe that $(g\tensor h)\tau_a = \tau_{g(a)} h$, from which~(1) follows routinely.
To show~(2), first assume by~(1) that w.l.o.g.\ $h=\id$ and $u=\id$. Then~(2) follows 
from the calculation
%
\begin{flalign*}
&&\sum\nolimits_{i,j} \norm{f(g(e_j'), e_i)}^2 
=&\;\sum\nolimits_{j} \norm{f\comp\tau_{g(e_j')}}_2^2\\
&&\leq &\;\sum\nolimits_{j} c^2\norm{g(e_j')}^2&\by{boundedness of $a\mto f\comp\tau_a$}\\
&&\leq &\;c^2 c'^2.&\by{for $g$ is H-S}
\end{flalign*} 
where $(e_i)_i$ and $(e_j')_j$ are some orthonormal bases in $X$ and $V'$ respectively.

Finally, let us show~(3). Again, by~(1), w.l.o.g.\ assume that $u=\id$ and $g=\id$. 
Clearly, for any $a\in V$, $f(\id\tensor h)\comp\tau_a = (f\tau_a)\comp h$ is Hilbert-Schmidt.
Let $(e_i)_i$ be an orthonormal basis in $X'$. Then for suitable $c$ and $c'$,
%
\begin{align*}
\norm{f(\id\tensor h)\comp\tau_a}_2^2
=\;&\sum\nolimits_i \norm{f(a, h(e_i))}^2\\
\leq\;& \sum\nolimits_i c^2\norm{h(e_i)}^2\comp\norm{a}^2\\
\leq\;& c^2 c'^2\norm{a}^2.
\end{align*}
and hence $\norm{f(\id\tensor h)\comp\tau_a}_2\leq c\comp c'\comp\norm{a}$.
\end{proof}
%
\begin{lemma}\label{lem:q-hs-comp}
Let $f\in\HS_V(X,U)$ and $g\in\HS_U(Y,Z)$. Then $g\comp (f\tensor\id)\comp\alpha_{V,X,Y}^\mone\in\HS_V(X\tensor Y,Z)$.
\end{lemma}
\begin{proof}
Since $g\comp (f\tensor\id)\comp\alpha_{V,X,Y}^\mone\comp\tau_a = g\comp (f\comp\tau_a\tensor\id)$,
condition~(i) of Definition~\ref{defn:p-hs} follows from Lemma~\ref{lem:q-hs-nat}~(1).
To establish condition~(ii), let us fix some orthonormal bases $(e_i)_i$ and $(e_j')_j$ 
in $X$ and $Y$ respectively. Then
%
\begin{align*}
\norm{g\comp (f\tensor\id)\comp\alpha_{V,X,Y}^\mone\comp\tau_a}_2^2
=\;&\norm{g\comp (f\comp\tau_a\tensor\id)}_2^2\\
=\;&\sum\nolimits_{i,j} \norm{g(f(e_i\tensor a)\tensor e_j')}^2\\
=\;&\sum\nolimits_{i,j} \norm{(g\comp \tau_{f(e_i\tensor a)})(e_j')}^2\\
=\;&\sum\nolimits_{i} \norm{g\comp \tau_{f(e_i\tensor a)}}^2_2\\
\leq\;&\sum\nolimits_{i} c^2\norm{f(e_i\tensor a)}^2\\
\leq\;&\sum\nolimits_{i} c^2\norm{(f\tau_a)(e_i)}^2\\
\leq\;&c'^2\comp c^2\comp\norm{a}.
\end{align*}   
for suitable $c$ and $c'$, and hence 
$g\comp (f\tensor\id)\comp\alpha_{V,X,Y}^\mone\comp\tau_a\leq c\comp c'\comp\norm{a}$.
\end{proof}

